Simulating metal complex formation and dynamics in aqueous solutions: Insights into stability, mechanism, and rates of ligand exchange

Metal coordination is ubiquitous in Nature and central in many applications ranging from nanotechnology to catalysis and environmental chemistry. Complex formation results from the subtle interplay between different thermodynamic, kinetic, and mechanistic contributions, which remain largely elusive to standard experimental methodologies and challenging for typical modeling approaches. Here, we present an effective molecular simulation approach that can fully describe the chemical equilibrium and dynamics of metal complexes in solution, with atomistic detail. Application to Cd(II) and Ni(II) complexes with various amine ligands provides an excellent agreement with available association constants and formation rates spanning several orders of magnitude. Moreover, investigation of polydentate ligands allows unravelling the origin of the chelate effect as due to the concurrent contribution of entropy, dissociation rates, and ligand binding mechanisms. This study represents a step forward for the in silico design of coordination chemistry applications and for a better understanding of biochemical processes activated by metal binding.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> xx.tex <==



==> xx2.tex <==


